Towards Family-Grouped Hierarchical Federated Learning on Sub-5KB Models: A Feasibility Study of Privacy-Preserving ECG Monitoring for Ultra-Resource-Constrained Wearables

Cardiovascular disease remains the leading cause of death worldwide, and early detection of arrhythmias through continuous ECG monitoring on wearable devices can prevent life-threatening events. Federated Learning (FL) enables privacy-preserving collaborative training by keeping raw ECG data on device, yet standard FL incurs prohibitive communication overhead and standard deep learning models cannot fit on ultra-low-power microcontrollers. We propose Family-Grouped Hierarchical Federated Learning (Family-FL), a three-tier architecture that uses the family as a natural privacy boundary for intra-family aggregation before global synchronization. We further design a hardware-constrained Tiny CNN-LSTM architecture with only 669 parameters, INT8-quantized to occupy merely 4.65KB Flash and 2.95KB RAM, meeting the constraints of STC32G12K128-class microcontrollers. Experiments on the MIT-BIH Arrhythmia Database (mean of 5 independent runs with different seeds) demonstrate that Family-FL reduces communication volume by 76.7% compared to FedAvg while maintaining comparable accuracy. Family-FL-Tiny achieves 91.9 +/- 1.2% accuracy with macro-F1 of 0.483 +/- 0.031, reducing total communication to 0.31% of FedAvg. The model achieves reliable ventricular arrhythmia detection (per-class F1 = 0.80), the most clinically critical abnormality for home-based preliminary screening. These results demonstrate the technical feasibility of privacy-preserving federated learning on ultra-resource-constrained microcontrollers through simulation-based evaluation. We honestly discuss limitations: no hardware deployment, single-dataset validation (MIT-BIH, 47 subjects), reduced rare-class sensitivity, and absence of formal differential privacy guarantees.

==> figures/fig1_architecture.tex <==
% Figure 1: Three-tier System Architecture
% Cloud Server (top) -> Home Hubs (middle) -> Wearable Devices (bottom)

\begin{tikzpicture}[
    node distance=1.2cm,
    server/.style={rectangle, draw, fill=blue!15, minimum width=3.5cm, minimum height=0.8cm, align=center, font=\small},
    hub/.style={rectangle, draw, fill=orange!15, minimum width=2.8cm, minimum height=0.7cm, align=center, font=\small},
    device/.style={rectangle, draw, fill=green!15, minimum width=2.2cm, minimum height=0.6cm, align=center, font=\footnotesize},
    arrow/.style={->, >=stealth, thick},
    label/.style={font=\footnotesize\bfseries}
]

% === Tier 1: Cloud Server ===
\node[server] (cloud) {Cloud Server\\[-2pt]\footnotesize(Global Model Aggregation)};
\node[label, left=0.3cm of cloud] (tier1) {Tier 1};

% === Tier 2: Home Hubs ===
\node[hub, below left=1.0cm and 0.6cm of cloud] (hub1) {Home Hub $H_1$\\[-2pt]\footnotesize(Local Aggregation)};
\node[hub, below=0.4cm of cloud] (hub2) {Home Hub $H_2$\\[-2pt]\footnotesize(Local Aggregation)};
\node[hub, below right=1.0cm and 0.6cm of cloud] (hub3) {Home Hub $H_3$};
\node[label, left=0.3cm of hub1] (tier2) {Tier 2};

% === Tier 3: Wearable Devices ===
\node[device, below left=0.7cm and 0.1cm of hub1] (dev1) {Device $d_{1,1}$};
\node[device, below right=0.7cm and 0.1cm of hub1] (dev2) {Device $d_{1,2}$};

\node[device, below=0.6cm of hub2] (dev3) {Device $d_{2,1}$};

\node[device, below left=0.7cm and 0.1cm of hub3] (dev4) {Device $d_{3,1}$};
\node[device, below right=0.7cm and 0.1cm of hub3] (dev5) {Device $d_{3,2}$};
\node[label, left=0.3cm of dev1] (tier3) {Tier 3};

% === Arrows: Cloud <-> Hubs ===
\draw[arrow, blue!60!black] (cloud) -- (hub1) node[midway, above, sloped, font=\tiny] {$\mathbf{w}_g$};
\draw[arrow, blue!60!black] (cloud) -- (hub2) node[midway, right, font=\tiny] {$\mathbf{w}_g$};
\draw[arrow, blue!60!black] (cloud) -- (hub3) node[midway, above, sloped, font=\tiny] {$\mathbf{w}_g$};

% === Arrows: Hubs <-> Devices ===
\draw[arrow, orange!70!black] (hub1) -- (dev1);
\draw[arrow, orange!70!black] (hub1) -- (dev2);
\draw[arrow, orange!70!black] (hub2) -- (dev3);
\draw[arrow, orange!70!black] (hub3) -- (dev4);
\draw[arrow, orange!70!black] (hub3) -- (dev5);

% === Legend ===
\node[anchor=south west, font=\footnotesize, align=left] at (4.5, -3.8) {
    \textcolor{blue!60!black}{$\mathbf{w}_g$}: Global model parameters\\
    \textcolor{orange!70!black}{$\mathbf{w}_l$}: Local model parameters
};

\end{tikzpicture}


==> figures/latex_includes.tex <==
%% LaTeX Include File for All Figures
%% Place \input{figures/latex_includes.tex} in your main document
%% or copy individual figure environments as needed.

%% ============================================================
%% Figure 1: Three-tier System Architecture (TikZ)
%% ============================================================
\begin{figure}[t]
    \centering
    \input{figures/fig1_architecture.tex}
    \caption{The three-tier \textcolor{black}{Family-FL} system architecture: Tier 1 (Cloud Server) maintains the global model; Tier 2 (Home Hubs) performs intra-family local aggregation; Tier 3 (Wearable Devices) collects personal health data and trains tiny on-device models.}
    \label{fig:architecture}
\end{figure}

%% ============================================================
%% Figure 2: TinyCNN-LSTM Model Architecture (TikZ)
%% ============================================================
\begin{figure}[t]
    \centering
    \input{figures/fig2_model_architecture.tex}
    \caption{The TinyCNN-LSTM model architecture designed for STM32-class microcontrollers. The network consists of a Conv1D feature extractor, an LSTM temporal module, and a fully-connected classifier, totaling only 637 parameters (4.7~KB Flash, 3.0~KB RAM).}
    \label{fig:model_architecture}
\end{figure}

%% ============================================================
%% Figure 3: Convergence Curves (PDF)
%% ============================================================
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/fig3_convergence.pdf}
    \caption{Test accuracy convergence over communication rounds. Centralized-LSTM (dashed line) reaches 98.0\% accuracy with no communication cost. Family-FL-Tiny converges to 91.9\% within 24 rounds, demonstrating feasible convergence for resource-constrained deployments.}
    \label{fig:convergence}
\end{figure}

%% ============================================================
%% Figure 4: Resource Comparison (PDF)
%% ============================================================
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/fig4_resource_comparison.pdf}
    \caption{Flash memory and RAM usage comparison across methods. The red dashed line indicates the STM32L010K4 resource limit (128~KB Flash / 12~KB RAM). Only Family-FL-Tiny fits within the MCU constraint, achieving \textbf{43.5$\times$} Flash and \textbf{407$\times$} RAM reduction over baselines.}
    \label{fig:resource_comparison}
\end{figure}

%% ============================================================
%% Figure 5: Communication Cost (PDF)
%% ============================================================
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/fig5_communication.pdf}
    \caption{Total communication cost per device over the entire training process. Family-FL reduces communication by 76.8\% compared to FedAvg; Family-FL-Tiny achieves a \textbf{99.7\%} reduction, lowering the cost from 853~MB to only 2.6~KB.}
    \label{fig:communication}
\end{figure}

%% ============================================================
%% Figure 6: Accuracy vs Communication Tradeoff (PDF)
%% ============================================================
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/fig6_accuracy_comm_tradeoff.pdf}
    \caption{Accuracy--communication tradeoff. Family-FL-Tiny (Ours) achieves Pareto optimality for resource-constrained deployments, reducing communication by 99.7\% with only 4.5\% accuracy degradation compared to Family-FL.}
    \label{fig:tradeoff}
\end{figure}

%% ============================================================
%% Figure 7: Confusion Matrix (NEW - Per-class prediction analysis)
%% ============================================================
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/fig7_confusion_matrix.pdf}
    \caption{Normalized confusion matrix for Family-FL-Tiny (best run, seed=42). The model excels at Normal (N) classification (99\% recall) and achieves reasonable Ventricular (V) detection (82\% recall), but struggles with rare classes: Supraventricular (S, 38\% recall), Fusion (F, 8\% recall), and Unclassified (Q, 18\% recall). Values are row-normalized (recall per true class).}
    \label{fig:confusion_matrix}
\end{figure}

%% ============================================================
%% Figure 8: Per-Class F1 Comparison (NEW)
%% ============================================================
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/fig8_per_class_f1.pdf}
    \caption{Per-class F1-score comparison across all methods. All full-size methods (Centralized, FedAvg, FedProx, Family-FL) achieve strong performance across all classes. Tiny models (FedAvg-Tiny, Family-FL-Tiny) show severe degradation on rare classes (S, F, Q) due to limited model capacity, while maintaining reasonable performance on N and V classes. Family-FL-Tiny marginally outperforms FedAvg-Tiny on most classes, reflecting the benefit of family-grouped aggregation.}
    \label{fig:per_class_f1}
\end{figure}

